Fast simulation of muons produced at the SHiP experiment using Generative Adversarial Networks

This paper presents a fast approach to simulating muons produced in interactions of the SPS proton beams with the target of the SHiP experiment. The SHiP experiment will be able to search for new long-lived particles produced in a 400~GeV$/c$ SPS proton beam dump and which travel distances between fifty metres and tens of kilometers. The SHiP detector needs to operate under ultra-low background conditions and requires large simulated samples of muon induced background processes. Through the use of Generative Adversarial Networks it is possible to emulate the simulation of the interaction of 400~GeV$/c$ proton beams with the SHiP target, an otherwise computationally intensive process. For the simulation requirements of the SHiP experiment, generative networks are capable of approximating the full simulation of the dense fixed target, offering a speed increase by a factor of $\mathcal{O}(10^6)$. To evaluate the performance of such an approach, comparisons of the distributions of reconstructed muon momenta in SHiP's spectrometer between samples using the full simulation and samples produced through generative models are presented. The methods discussed in this paper can be generalised and applied to modelling any non-discrete multi-dimensional distribution.

==> authors_pre.tex <==

\begin{flushleft}
%-- 
%-- SHiP Authorlist as of 15 August 2019
%-- 
C.~Ahdida$^{44}$,
R.~Albanese$^{14,d,h}$,
A.~Alexandrov$^{14}$,
A.~Anokhina$^{39}$,
S.~Aoki$^{18}$,
G.~Arduini$^{44}$,
E.~Atkin$^{38}$,
N.~Azorskiy$^{29}$,
J.J.~Back$^{54}$,
A.~Bagulya$^{32}$,
F.~Baaltasar~Dos~Santos$^{44}$,
A.~Baranov$^{40}$,
F.~Bardou$^{44}$,
G.J.~Barker$^{54}$,
M.~Battistin$^{44}$,
J.~Bauche$^{44}$,
A.~Bay$^{46}$,
V.~Bayliss$^{51}$,
G.~Bencivenni$^{15}$,
A.Y.~Berdnikov$^{37}$,
Y.A.~Berdnikov$^{37}$,
I.~Berezkina$^{32}$,
M.~Bertani$^{15}$,
C.~Betancourt$^{47}$,
I.~Bezshyiko$^{47}$,
O.~Bezshyyko$^{55}$,
D.~Bick$^{8}$,
S.~Bieschke$^{8}$,
A.~Blanco$^{28}$,
J.~Boehm$^{51}$,
M.~Bogomilov$^{1}$,
K.~Bondarenko$^{27,57}$,
W.M.~Bonivento$^{13}$,
J.~Borburgh$^{44}$,
A.~Boyarsky$^{27,55}$,
R.~Brenner$^{43}$,
D.~Breton$^{4}$,
R.~Brundler$^{47}$,
M.~Bruschi$^{12}$,
V.~B\"{u}scher$^{10}$,
A.~Buonaura$^{47}$,
S.~Buontempo$^{14}$,
S.~Cadeddu$^{13}$,
A.~Calcaterra$^{15}$,
M.~Calviani$^{44}$,
M.~Campanelli$^{53}$,
M.~Casolino$^{44}$,
N.~Charitonidis$^{44}$,
P.~Chau$^{10}$,
J.~Chauveau$^{5}$,
A.~Chepurnov$^{39}$,
M.~Chernyavskiy$^{32}$,
K.-Y.~Choi$^{26}$,
A.~Chumakov$^{2}$,
P.~Ciambrone$^{15}$,
L.~Congedo$^{11,a}$,
K.~Cornelis$^{44}$,
M.~Cristinziani$^{7}$,
A.~Crupano$^{14,d}$,
G.M.~Dallavalle$^{12}$,
A.~Datwyler$^{47}$,
N.~D'Ambrosio$^{16}$,
G.~D'Appollonio$^{13,c}$,
J.~De~Carvalho~Saraiva$^{28}$,
G.~De~Lellis$^{14,34,44,d}$,
M.~de~Magistris$^{14,d}$,
A.~De~Roeck$^{44}$,
M.~De~Serio$^{11,a}$,
D.~De~Simone$^{14,d}$,
L.~Dedenko$^{39}$,
P.~Dergachev$^{34}$,
A.~Di~Crescenzo$^{14,d}$,
N.~Di~Marco$^{16}$,
C.~Dib$^{2}$,
H.~Dijkstra$^{44}$,
P.~Dipinto$^{11,a}$,
V.~Dmitrenko$^{38}$,
S.~Dmitrievskiy$^{29}$,
L.A.~Dougherty$^{44}$,
A.~Dolmatov$^{30}$,
D.~Domenici$^{15}$,
S.~Donskov$^{35}$,
V.~Drohan$^{55}$,
A.~Dubreuil$^{45}$,
M.~Ehlert$^{6}$,
T.~Enik$^{29}$,
A.~Etenko$^{33,38}$,
F.~Fabbri$^{12}$,
L.~Fabbri$^{12,b}$,
A.~Fabich$^{44}$,
O.~Fedin$^{36}$,
F.~Fedotovs$^{52}$,
G.~Felici$^{15}$,
M.~Ferro-Luzzi$^{44}$,
K.~Filippov$^{38}$,
R.A.~Fini$^{11}$,
P.~Fonte$^{28}$,
C.~Franco$^{28}$,
M.~Fraser$^{44}$,
R.~Fresa$^{14,i}$,
R.~Froeschl$^{44}$,
T.~Fukuda$^{19}$,
G.~Galati$^{14,d}$,
J.~Gall$^{44}$,
L.~Gatignon$^{44}$,
G.~Gavrilov$^{38}$,
V.~Gentile$^{14,d}$,
S.~Gerlach$^{6}$,
B.~Goddard$^{44}$,
L.~Golinka-Bezshyyko$^{55}$,
A.~Golovatiuk$^{14,d}$,
D.~Golubkov$^{30}$,
A.~Golutvin$^{52}$,
P.~Gorbounov$^{44}$,
D.~Gorbunov$^{31}$,
S.~Gorbunov$^{32}$,
V.~Gorkavenko$^{55}$,
Y.~Gornushkin$^{29}$,
M.~Gorshenkov$^{34}$,
V.~Grachev$^{38}$,
A.L.~Grandchamp$^{46}$,
G.~Granich$^{32}$,
E.~Graverini$^{46}$,
J.-L.~Grenard$^{44}$,
D.~Grenier$^{44}$,
V.~Grichine$^{32}$,
N.~Gruzinskii$^{36}$,
A.~M.~Guler$^{48}$,
Yu.~Guz$^{35}$,
G.J.~Haefeli$^{46}$,
C.~Hagner$^{8}$,
H.~Hakobyan$^{2}$,
I.W.~Harris$^{46}$,
E.~van~Herwijnen$^{44}$,
C.~Hessler$^{44}$,
A.~Hollnagel$^{10}$,
B.~Hosseini$^{52}$,
M.~Hushchyn$^{40}$,
G.~Iaselli$^{11,a}$,
A.~Iuliano$^{14,d}$,
V.~Ivantchenko$^{32}$,
R.~Jacobsson$^{44}$,
D.~Jokovi\'{c}$^{41}$,
M.~Jonker$^{44}$,
I.~Kadenko$^{55}$,
V.~Kain$^{44}$,
B.~Kaiser$^{8}$,
C.~Kamiscioglu$^{49}$,
K.~Kershaw$^{44}$,
M.~Khabibullin$^{31}$,
E.~Khalikov$^{39}$,
G.~Khaustov$^{35}$,
G.~Khoriauli$^{10}$,
A.~Khotyantsev$^{31}$,
S.H.~Kim$^{22}$,
Y.G.~Kim$^{23}$,
V.~Kim$^{36,37}$,
N.~Kitagawa$^{19}$,
J.-W.~Ko$^{22}$,
K.~Kodama$^{17}$,
A.~Kolesnikov$^{29}$,
D.I.~Kolev$^{1}$,
V.~Kolosov$^{35}$,
M.~Komatsu$^{19}$,
N.~Kondrateva$^{32}$,
A.~Kono$^{21}$,
N.~Konovalova$^{32,34}$,
S.~Kormannshaus$^{10}$,
I.~Korol$^{6}$,
I.~Korol'ko$^{30}$,
A.~Korzenev$^{45}$,
V.~Kostyukhin$^{7}$,
E.~Koukovini~Platia$^{44}$,
S.~Kovalenko$^{2}$,
I.~Krasilnikova$^{34}$,
Y.~Kudenko$^{31,38,g}$,
E.~Kurbatov$^{40}$,
P.~Kurbatov$^{34}$,
V.~Kurochka$^{31}$,
E.~Kuznetsova$^{36}$,
H.M.~Lacker$^{6}$,
M.~Lamont$^{44}$,
G.~Lanfranchi$^{15}$,
O.~Lantwin$^{52}$,
A.~Lauria$^{14,d}$,
K.S.~Lee$^{25}$,
K.Y.~Lee$^{22}$,
J.-M.~L\'{e}vy$^{5}$,
V.P.~Loschiavo$^{14,h}$,
L.~Lopes$^{28}$,
E.~Lopez~Sola$^{44}$,
V.~Lyubovitskij$^{2}$,
J.~Maalmi$^{4}$,
A.~Magnan$^{52}$,
V.~Maleev$^{36}$,
A.~Malinin$^{33}$,
Y.~Manabe$^{19}$,
A.K.~Managadze$^{39}$,
M.~Manfredi$^{44}$,
S.~Marsh$^{44}$,
A.M.~Marshall$^{50}$,
A.~Mefodev$^{31}$,
P.~Mermod$^{45}$,
A.~Miano$^{14,d}$,
S.~Mikado$^{20}$,
Yu.~Mikhaylov$^{35}$,
D.A.~Milstead$^{42}$,
O.~Mineev$^{31}$,
A.~Montanari$^{12}$,
M.C.~Montesi$^{14,d}$,
K.~Morishima$^{19}$,
S.~Movchan$^{29}$,
Y.~Muttoni$^{44}$,
N.~Naganawa$^{19}$,
M.~Nakamura$^{19}$,
T.~Nakano$^{19}$,
S.~Nasybulin$^{36}$,
P.~Ninin$^{44}$,
A.~Nishio$^{19}$,
A.~Novikov$^{38}$,
B.~Obinyakov$^{33}$,
S.~Ogawa$^{21}$,
N.~Okateva$^{32,34}$,
B.~Opitz$^{8}$,
J.~Osborne$^{44}$,
M.~Ovchynnikov$^{27,55}$,
N.~Owtscharenko$^{7}$,
P.H.~Owen$^{47}$,
P.~Pacholek$^{44}$,
A.~Paoloni$^{15}$,
B.D.~Park$^{22}$,
S.K.~Park$^{25}$,
A.~Pastore$^{11}$,
M.~Patel$^{52}$,
D.~Pereyma$^{30}$,
A.~Perillo-Marcone$^{44}$,
G.L.~Petkov$^{1}$,
K.~Petridis$^{50}$,
A.~Petrov$^{33}$,
D.~Podgrudkov$^{39}$,
V.~Poliakov$^{35}$,
N.~Polukhina$^{32,34,38}$,
J.~Prieto~Prieto$^{44}$,
M.~Prokudin$^{30}$,
A.~Prota$^{14,d}$,
A.~Quercia$^{14,d}$,
A.~Rademakers$^{44}$,
A.~Rakai$^{44}$,
F.~Ratnikov$^{40}$,
T.~Rawlings$^{51}$,
F.~Redi$^{46}$,
S.~Ricciardi$^{51}$,
M.~Rinaldesi$^{44}$,
Volodymyr~Rodin$^{55}$,
Viktor~Rodin$^{55}$,
P.~Robbe$^{4}$,
A.B.~Rodrigues~Cavalcante$^{46}$,
T.~Roganova$^{39}$,
H.~Rokujo$^{19}$,
G.~Rosa$^{14,d}$,
T.~Rovelli$^{12,b}$,
O.~Ruchayskiy$^{3}$,
T.~Ruf$^{44}$,
V.~Samoylenko$^{35}$,
V.~Samsonov$^{38}$,
F.~Sanchez~Galan$^{44}$,
P.~Santos~Diaz$^{44}$,
A.~Sanz~Ull$^{44}$,
A.~Saputi$^{15}$,
O.~Sato$^{19}$,
E.S.~Savchenko$^{34}$,
J.S.~Schliwinski$^{6}$,
W.~Schmidt-Parzefall$^{8}$,
N.~Serra$^{47}$,
S.~Sgobba$^{44}$,
O.~Shadura$^{55}$,
A.~Shakin$^{34}$,
M.~Shaposhnikov$^{46}$,
P.~Shatalov$^{30}$,
T.~Shchedrina$^{32,34}$,
L.~Shchutska$^{55}$,
V.~Shevchenko$^{33}$,
H.~Shibuya$^{21}$,
L.~Shihora$^{6}$,
S.~Shirobokov$^{52}$,
A.~Shustov$^{38}$,
S.B.~Silverstein$^{42}$,
S.~Simone$^{11,a}$,
R.~Simoniello$^{10}$,
M.~Skorokhvatov$^{38,33}$,
S.~Smirnov$^{38}$,
J.Y.~Sohn$^{22}$,
A.~Sokolenko$^{55}$,
E.~Solodko$^{44}$,
N.~Starkov$^{32,33}$,
L.~Stoel$^{44}$,
B.~Storaci$^{47}$,
M.E.~Stramaglia$^{46}$,
D.~Sukhonos$^{44}$,
Y.~Suzuki$^{19}$,
S.~Takahashi$^{18}$,
J.L.~Tastet$^{3}$,
P.~Teterin$^{38}$,
S.~Than~Naing$^{32}$,
I.~Timiryasov$^{46}$,
V.~Tioukov$^{14}$,
D.~Tommasini$^{44}$,
M.~Torii$^{19}$,
N.~Tosi$^{12}$,
D.~Treille$^{44}$,
R.~Tsenov$^{1,29}$,
S.~Ulin$^{38}$,
A.~Ustyuzhanin$^{40}$,
Z.~Uteshev$^{38}$,
G.~Vankova-Kirilova$^{1}$,
F.~Vannucci$^{5}$,
P.~Venkova$^{6}$,
V.~Venturi$^{44}$,
S.~Vilchinski$^{55}$,
M.~Villa$^{12,b}$,
Heinz~Vincke$^{44}$,
Helmut~Vincke$^{44}$,
C.~Visone$^{14,d}$,
K.~Vlasik$^{38}$,
A.~Volkov$^{32,33}$,
R.~Voronkov$^{32}$,
S.~van~Waasen$^{9}$,
R.~Wanke$^{10}$,
P.~Wertelaers$^{44}$,
J.-K.~Woo$^{24}$,
M.~Wurm$^{10}$,
S.~Xella$^{3}$,
D.~Yilmaz$^{49}$,
A.U.~Yilmazer$^{49}$,
C.S.~Yoon$^{22}$,
P.~Zarubin$^{29}$,
I.~Zarubina$^{29}$,
Yu.~Zaytsev$^{30}$

\vspace*{1cm}

{\footnotesize \it

$ ^{1}$Faculty of Physics, Sofia University, Sofia, Bulgaria\\
$ ^{2}$Universidad T\'ecnica Federico Santa Mar\'ia and Centro Cient\'ifico Tecnol\'ogico de Valpara\'iso, Valpara\'iso, Chile\\
$ ^{3}$Niels Bohr Institute, University of Copenhagen, Copenhagen, Denmark\\
$ ^{4}$LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit\'{e} Paris-Saclay, Orsay, France\\
$ ^{5}$LPNHE, IN2P3/CNRS, Sorbonne Universit\'{e}, Universit\'{e} Paris Diderot,F-75252 Paris, France\\
$ ^{6}$Humboldt-Universit\"{a}t zu Berlin, Berlin, Germany\\
$ ^{7}$Physikalisches Institut, Universit\"{a}t Bonn, Bonn, Germany\\
$ ^{8}$Universit\"{a}t Hamburg, Hamburg, Germany\\
$ ^{9}$Forschungszentrum J\"{u}lich GmbH (KFA),  J\"{u}lich , Germany\\
$ ^{10}$Institut f\"{u}r Physik and PRISMA Cluster of Excellence, Johannes Gutenberg Universit\"{a}t Mainz, Mainz, Germany\\
$ ^{11}$Sezione INFN di Bari, Bari, Italy\\
$ ^{12}$Sezione INFN di Bologna, Bologna, Italy\\
$ ^{13}$Sezione INFN di Cagliari, Cagliari, Italy\\
$ ^{14}$Sezione INFN di Napoli, Napoli, Italy\\
$ ^{15}$Laboratori Nazionali dell'INFN di Frascati, Frascati, Italy\\
$ ^{16}$Laboratori Nazionali dell'INFN di Gran Sasso, L'Aquila, Italy\\
$ ^{17}$Aichi University of Education, Kariya, Japan\\
$ ^{18}$Kobe University, Kobe, Japan\\
$ ^{19}$Nagoya University, Nagoya, Japan\\
$ ^{20}$College of Industrial Technology, Nihon University, Narashino, Japan\\
$ ^{21}$Toho University, Funabashi, Chiba, Japan\\
$ ^{22}$Physics Education Department \& RINS, Gyeongsang National University, Jinju, Korea\\
$ ^{23}$Gwangju National University of Education~$^{e}$, Gwangju, Korea\\
$ ^{24}$Jeju National University~$^{e}$, Jeju, Korea\\
$ ^{25}$Korea University, Seoul, Korea\\
$ ^{26}$Sungkyunkwan University~$^{e}$, Suwon-si, Gyeong Gi-do, Korea\\
$ ^{27}$University of Leiden, Leiden, The Netherlands\\
$ ^{28}$LIP, Laboratory of Instrumentation and Experimental Particle Physics, Portugal\\
$ ^{29}$Joint Institute for Nuclear Research (JINR), Dubna, Russia\\
$ ^{30}$Institute of Theoretical and Experimental Physics (ITEP) NRC 'Kurchatov Institute', Moscow, Russia\\
$ ^{31}$Institute for Nuclear Research of the Russian Academy of Sciences (INR RAS), Moscow, Russia\\
$ ^{32}$P.N.~Lebedev Physical Institute (LPI), Moscow, Russia\\
$ ^{33}$National Research Centre 'Kurchatov Institute', Moscow, Russia\\
$ ^{34}$National University of Science and Technology "MISiS", Moscow, Russia\\
$ ^{35}$Institute for High Energy Physics (IHEP) NRC 'Kurchatov Institute', Protvino, Russia\\
$ ^{36}$Petersburg Nuclear Physics Institute (PNPI) NRC 'Kurchatov Institute', Gatchina, Russia\\
$ ^{37}$St. Petersburg Polytechnic University (SPbPU)~$^{f}$, St. Petersburg, Russia\\
$ ^{38}$National Research Nuclear University (MEPhI), Moscow, Russia\\
$ ^{39}$Skobeltsyn Institute of Nuclear Physics of Moscow State University (SINP MSU), Moscow, Russia\\
$ ^{40}$Yandex School of Data Analysis, Moscow, Russia\\
$ ^{41}$Institute of Physics, University of Belgrade, Serbia\\
$ ^{42}$Stockholm University, Stockholm, Sweden\\
$ ^{43}$Uppsala University, Uppsala, Sweden\\
$ ^{44}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$ ^{45}$University of Geneva, Geneva, Switzerland\\
$ ^{46}$\'{E}cole Polytechnique F\'{e}d\'{e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$ ^{47}$Physik-Institut, Universit\"{a}t Z\"{u}rich, Z\"{u}rich, Switzerland\\
$ ^{48}$Middle East Technical University (METU), Ankara, Turkey\\
$ ^{49}$Ankara University, Ankara, Turkey\\
$ ^{50}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom \\
$ ^{51}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$ ^{52}$Imperial College London, London, United Kingdom\\
$ ^{53}$University College London, London, United Kingdom\\
$ ^{54}$University of Warwick, Warwick, United Kingdom\\
$ ^{55}$Taras Shevchenko National University of Kyiv, Kyiv, Ukraine\\
$ ^{a}$Universit\`{a} di Bari, Bari, Italy\\
$ ^{b}$Universit\`{a} di Bologna, Bologna, Italy\\
$ ^{c}$Universit\`{a} di Cagliari, Cagliari, Italy\\
$ ^{d}$Universit\`{a} di Napoli ``Federico II'', Napoli, Italy\\
$ ^{e}$Associated to Gyeongsang National University, Jinju, Korea\\
$ ^{f}$Associated to Petersburg Nuclear Physics Institute (PNPI), Gatchina, Russia\\
$ ^{g}$Also at Moscow Institute of Physics and Technology (MIPT),  Moscow Region, Russia\\
$ ^{h}$Consorzio CREATE, Napoli, Italy\\
$ ^{i}$Universit\`{a} della Basilicata, Potenza, Italy\\
}
\end{flushleft}




